Deletion Inference, Reconstruction, and Compliance in Machine (Un)Learning

Privacy attacks on machine learning models aim to identify the data that is used to train such models. Such attacks, traditionally, are studied on static models that are trained once and are accessible by the adversary. Motivated to meet new legal requirements, many machine learning methods are recently extended to support machine unlearning, i.e., updating models as if certain examples are removed from their training sets, and meet new legal requirements. However, privacy attacks could potentially become more devastating in this new setting, since an attacker could now access both the original model before deletion and the new model after the deletion. In fact, the very act of deletion might make the deleted record more vulnerable to privacy attacks. Inspired by cryptographic definitions and the differential privacy framework, we formally study privacy implications of machine unlearning. We formalize (various forms of) deletion inference and deletion reconstruction attacks, in which the adversary aims to either identify which record is deleted or to reconstruct (perhaps part of) the deleted records. We then present successful deletion inference and reconstruction attacks for a variety of machine learning models and tasks such as classification, regression, and language models. Finally, we show that our attacks would provably be precluded if the schemes satisfy (variants of) Deletion Compliance (Garg, Goldwasser, and Vasudevan, Eurocrypt' 20).

==> CompareMembership.tex <==
{
\section{Comparison with Reduction to the MI Attack of \cite{yeom2018privacy}} \label{sec:CompareApp}
 
Additionally, here we compare our direct deletion inference attack $\DInfWith$ with a reduction (as stated in Algorithm~\ref{const:reduction_adversary}) to membership inference attacks of Yeom et al.~\cite{yeom2018privacy}.  
%In particular, we first obtain deletion inference by using the reduction of Algorithm~\ref{const:reduction_adversary} to the membership inference attack of \cite{yeom2018privacy}, and then we compare the findings  with our own attack $\DInfWith$.
 %As a directly comparable baseline to $\DInfWith$, 
% 
The membership inference adversary of Yeom et al.~\cite{yeom2018privacy}  works with a threshold value that is chosen to be the average of losses over all the training examples as an auxiliary information. This threshold can   be estimated by the adversary from extra examples sampled from the distribution. The adversary predicts an example to be a member of the model if the loss of that example is smaller than the average training loss.  
 We use the original code, models, and data released by~\cite{yeom2018privacy}. Specifically, we use two datasets IWPC (International Warfarin Pharmacogenetics Consortium) \cite{international2009estimation} and Eyedata \cite{scheetz2006regulation} from~\cite{yeom2018privacy}. The statistics of the datasets are summarized in Table~\ref{tab:dataset}. Regarding the hyperparameters, we report the success probability of both attacks on the model with best performance without attack, which is selected via cross validation. The experiment's results are shown in Table~\ref{tab:reduct_delinf}. 
 
 Our simple adversary algorithms achieve around 90\% success probability in almost all cases, in both settings  of  comparing with samples in the training set (inside $\cS$)  or comparing with samples outside the training dataset (outside $\cS$). In most cases, the success in fact close to $100\%$. Clearly, with the access of both versions of models, there exists an obvious privacy leak that can be easily exploited by naive adversaries.%, even when the deletion is perfect.
% \Jnote{ToDo: Improve the result by choosing a different parameter}


% \begin{compactitem}
%     \item \textbf{Data Generation}: 
%     % We repeat the adversarial experiment $\text{RemEx}$ by 1000 runs.  Each run we randomly draw one sample $(x_e, y_e)$ from the training dataset to delete, and draw an additional sample following the experiment protocol. The success criteria of the experiment is the success probability of 
%     % both adversary experiments $\text{RemEx}$ and $\text{RemExL}$.
% \end{compactitem}



\begin{table}[ht]
% \scriptsize
\centering
\begin{tabular}{lll}
\hline
        & \multicolumn{1}{c}{Reduction to Mem. Inf.}                              & \multicolumn{1}{c}{$\DInfWith$}                                         \\ \hline
        % & \multicolumn{1}{c}{Inside $\cS$} & \multicolumn{1}{c}{Outside $\cS$} & \multicolumn{1}{c}{Inside $\cS$} & \multicolumn{1}{c}{Outside $\cS$} \\ \hline
Eyedata & 64.80\%                                                & 97.54\%                                                    \\ \hline
IWPC    & 68.83\%                                                 & 95.98\%                                                    \\ \hline
\end{tabular}
% \captionsetup{justification=centering}
\caption{Comparing the success probabilities  of our attack  $\DInfWith$ and an alternative attack based on reduction to the membership inference attack of Yeom et al.~\cite{yeom2018privacy}.}
\label{tab:reduct_delinf}
\end{table}
% \paragraph{Experiments' results.} We present the success probability result of the experiments in Table~\ref{tab:res_regression}. Our simple adversary algorithms achieve around 90\% success probability in almost all cases, in both settings  of  comparing with samples in the training set (inside $\cS$)  or comparing with samples outside the training dataset (outside $\cS$). In most cases, the success in fact close to $100\%$.

%Clearly, with the access of both versions of models, there exists an obvious privacy leak that can be easily exploited by naive adversaries, even when the deletion is perfect.

}

==> Conclusion.tex <==
\section{Conclusion} 
%\Mnote{In light of space limitations and the fact that reviewers have already reviewed our paper, this section is optional in my opinion.}
In this work, we presented various attacks that infer or extract information about the deleted examples for a machine learning scheme with unlearning capability.
Our various leakage attacks demonstrate that the unlearning operation could come at an extra cost in privacy loss. In particular, we introduced \emph{deletion inference} and \emph{deletion reconstruction} attacks that are reminiscent of membership and data reconstruction attacks in the traditional setting where no updates are applied to the model. One remedy to prevent such leakage  is to use a \emph{deletion compliant} scheme, as defined in \cite{GGV20}, which can be realized from     forms of differential privacy~\cite{DNPR10,JKT12,CSS10}.
%
Many   intriguing questions remain open. Most prominently, it remains open to find \emph{efficient} learning methods with high accuracy that allow deletion with provable privacy guarantees. 


==> DelComp.tex <==
\section{Deletion Compliance for Machine (Un)Learning}
\label{sec:del-comp}


%We start by defining a variant of the notion of deletion-compliance of Garg, Goldwasser and Vasudevan~\cite{GGV20}, called \emph{weak deletion-compliance}, that naturally accommodates the above adversarial setting and clearly rules out the kinds of attacks we demonstrated. We then ask what algorithms can satisfy this definition. Towards answering this, we consider the notion of differential privacy under continual observation~\cite{DNPR10} and identify a specialization of it that is suited for our purposes, which we call  $k$-deletion privacy. We finally show how to use $k$-deletion privacy to construct such weak deletion-compliant machine learning systems. 

%\paragraph{Universe of records.} 







\Mnote{have not finished section below.}
\subsection{Weak deletion Compliance from Differential Privacy}
\label{sec:dp-cont}

The notion of differential privacy under continual observation was formulated by Dwork et al.~\cite{DNPR10} to capture privacy in settings where accesses to a system might happen at different points in its execution (see also \cite{CSS10} and \cite{JKT12} for similar but more specific definitions). They consider a streaming algorithm $\Alg$ that is given a stream $\vec{x} = (x_1, \dots, x_n)$ of inputs, where each $x_i$ is from a universe $\cX$. On receiving input $x_i$ in the stream, $\Alg$ produces an output $y_i$, resulting in a sequence of outputs $\vec{y}$. Two streams $\vec{x}$ and $\vec{x}'$ are considered adjacent if both are the same length and there is at most one $i$ such that $x_i \neq x_i'$.\footnote{This is the special case of ``event-level'' adjacency. They also consider ``user-level'' adjacency where any number of occurrences of a single element in the stream may be replaced by those of another element.} Denote by $\cY$ the universe of output sequences. Their definition is as follows.

\begin{definition}[DP under continual observation]
    \label{def:continual-dp}
    An algorithm $\Alg$ mapping streams from $\cX^*$ to an output sequence from $\cY$ is \emph{event-level $\eps$-private} for an $\eps\in\reals^+$ if for all $Y \subseteq \cY$, and all pairs of adjacent streams $\vec{x},\vec{x}'$,
    \begin{align*}
      \pr{\Alg(\vec{x}) \in Y} \leq e^{\eps} \cdot \pr{\Alg(\vec{x}') \in Y}
    \end{align*}
\end{definition}

When applied to a learning algorithm with the stream of inputs representing deletion requests and the output representing the updated models, such a notion of privacy would seem to provide us with the kind of privacy we are looking for, where the deleted data is private even given access to the models at various points. Below, we isolate this special case of this definition tailored to support a limited number of deletions.

\begin{definition}[$k$-deletion privacy] \label{def:StrongDelPriv}
Let $\Learn$ be a learning algorithm, $\Del$ be a removal/deletion mechanism for $\Learn$, and  $\DataCol$ be a distribution over $\cX \times \cY$ (the set of instances and labels).
For sample complexity $n$ and deletion budget $k \leq n$, consider the following experiment played between the adversary $A$ and challenger $C$.
\begin{itemize}
    \item {\bf Picking the data set.} Adversary picks $\set{e_1,\dots,e_n}$ from $\Supp(D)^n$.
    \item {\bf Picking the deletion sequences.} Adversary picks two sequences $\bfd= (d^0_1,\dots,d^0_k)$ and $\bfd'=(d^1_1,\dots,d^1_k)$ where: 
    \begin{enumerate}
        \item All $d^b_j \in \cS$ are potential examples to be deleted from $\cS$.
        \item Both sequences consist of distinct elements. Namely, for all $c \in \bits,i \neq j \in [k]$, we have $d^c_i \neq d^c_j$.
        \item For all but at most one $i \in [n]$, the sequences are the same. Namely, there is $i \in [k]$ such that for all $j \in [k], j \neq i$, it holds that $d^0_j = d^1_j$.
    \end{enumerate}
    \item {\bf Computing the deletions.}  Let $h_n \gets \Learn(\cS)$ be the original model before deletions start. The challenger picks $b \gets \bits $ at random. 
    For $i=1,2,\dots,k$ (inductively) let $h_{n-i} \gets \Del(h_{n-i+1},d^b_i)$.\footnote{The deletion operation might need extra data set stored in addition to the model for the sake of efficiency.} 
%    \item {\bf Adversary's guess.}  The adversary gets access to all of $h_{n},\dots,h_{n-k}$ and outputs bit  $b'$. The output of the experiment is defined to be $1$ (called win for the adversary) if $b'=b$, and $0$ otherwise.
\end{itemize}
We call the deletion scheme $\eps(n)$ differentially private for $k$ deletions, if for all such adversaries, all $\vec{h}$, and both bits $\beta \in \bits$ it holds that
\begin{equation*}
\begin{split}
   &\Pr[(h_{n},\dots,h_{n-k}) = \vec{h} \mid b=\beta]  \\
&\leq e^\eps \cdot \Pr[(h_{n},\dots,h_{n-k}) = \vec{h} \mid b=1-\beta].      
\end{split}
\end{equation*}
\end{definition}


Definition~\ref{def:StrongDelPriv} represents a weaker version of \cref{def:continual-dp} in the desired specialized setting. It is specialized because it is specifically about (learning) algorithms that are initialized with a set of elements $\set{e_1,\dots,e_n}$ from a universe $\cX\times\cY$, and the subsequent stream of inputs consists of deletion requests for some of these $e_i$'s. It is weaker because it bounds the lengths of the input streams by $k$.



\paragraph{Deletion compliant machine unlearning.} Finally, we observe that any learning algorithm that has a deletion mechanism satisfying $k$-deletion privacy (\cref{def:StrongDelPriv}) can be used to realize a Weak deletion-compliant data collector that maintains a model learned with this algorithm from its collected data.

Consider a data collector $\textsf{Learner}$ that uses a pair of algorithms $(\Learn,\Del)$ and works as follows:
\begin{itemize}[itemsep=0pt,topsep=5pt]
  \item It is initialized with an empty database $S$ and a ``threshold'' $n\in\N$.
  \item When a user submits a record $e$ to the collector, it inserts $e$ into the database $S$.
  \item The first time it has $n$ entries in its database, it runs $\Learn(S)$ to compute the model $h$ and stores it.
  \item When a user asks for its record $e$ to be deleted, it updates $h$ (if it exists) as $h \gets \Del(h,e)$, and also deletes $e$ from $S$.
  \item When a user makes a query $x$, if $h$ exists, it returns $h(x)$.
\end{itemize}

Further, suppose the collector interacts with its users over properly authenticated channels, and uses a \emph{history-independent} data structure\footnote{A history-independent implementation of a data structure, as defined in \cite{Mic97,NT01}, is one where the representation of the data structure in memory at any point depends only on the logical content of the data structure at that point. Such implementations are crucial to avoid side-effects in the course of deletion, and to achieve deletion-compliance~\cite{GGV20}.} to maintain the database $S$. Then, the following can be shown using arguments similar to those in \cite{GGV20}.

\begin{inftheorem}
    \label{infthm:del-comp}
    Under the conditions of authentication and history-independence specified above, if $(\Learn,\Del)$ is $\eps$-differentially private for $k$ deletions, then the mechanism $\mathsf{Learner}$ is $\eps$-Weak deletion-compliant for up to $k$ deletions.
\end{inftheorem}



==> GGV-Compare.tex <==



\section{More on Deletion Compliance} \label{sec:GGV-relation}



==> MoreExp.tex <==
{ \color{blue}{}
\section{Reconstruction Experiments for Uniform Singletons}
% \Mnote{we can perhaps move this subsubsection to appendix.}
\paragraph{} We uniformly sample all the centers $x_i$. We repeat the experiment  for every example in the set (i.e., $n$ times where $n$ is the size of the training set).  In the experiment, we let $d = n$ range from $50$ to $250$, and we use $m = n^2$ samples by the adversary. 

\paragraph{Results.} 
% \Mnote{maybe we can call this paragraph something else? the whole subsection is about experiments. so not sure what is the optimal choice here. Also, it might be good to avoid the "precision goes down" image. Maybe we can always pick the number of samples and dimension both to be $n$, to somehow model the "large dimension" scenario. And then we can increase $n$ that increases both. In that case, I think the expected accuracy and success  accuracy stays on top, and maybe even gets better?}
The result for this experiment is displayed in Figure~\ref{fig:recon_singleton}. When $d=n=250$ our adversary gets a nearly perfect $99\%$ expected accuracy in its deletion reconstruction task, indicating a huge leakage in data privacy. Furthermore, when $n$ increases, the result gradually converges to $100\%$. This result shows that the vulnerability is not limited to the small dataset. The learning algorithm can be more vulnerable with a larger sample complexity $n$.

% \begin{table}[ht]
% \begin{tabular}{ll}
% \hline
% Accuracy & Avg. Correct Indices \\ \hline
% 95\%     & 99.95\%              \\ \hline
% \end{tabular}
% \caption{Result on Singleton Experiment.}
% \label{tab:recon_singleton}
% \end{table}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{Figures/exp1.pdf}
    \caption{Adversary's performance (Y-axis) versus sample complexity $n$ (X-axis) in the singleton setting using nearest neighbor models on random inputs from $\bits^d$. In the experiment, we let $d=n$ and $m=n^2$, where $n$ is the sample complexity, $d$ is the dimension and $m$ is the number of auxiliary inputs.  The blue curve shows the largest $\rho$ where the attack is a $(\rho, 1 -\rho)$-successful deletion reconstruction attack, and the orange curve shows the expected accuracy (defined in Definition~\ref{def:Del-Recon}).}
    \label{fig:recon_singleton}
\end{figure}

\section{Deleted Image Reconstruction for $1$-NN on Singletons}
% We run the security game of Definition~\ref{def:Del-Recon} with $100$ different random images from the dataset as the deleted image.
Here we examine the case when every class in the dataset is indeed singleton.

\paragraph{Results.} 
For $50$ out of the $100$ images, the adversary can find image that has label changed and make reconstruction. The result of this simple deletion reconstruction is shown in Figure~\ref{fig:recon_fig}. The result shows that this simple adversary successfully reconstructs the majority of the examples in the dataset in a visually recognizable way. { More concretely, $39$ out of the $50$ images in the image get the correct label when fed into the nearest neighbor classifier.}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.38\textwidth]{Figures/omniglot_v2.png}
    \caption{$50$ reconstructed images on Omniglot dataset. For each pair of images, the upper row is the reconstructed example, while the lower row is the actual deleted example.}
    \label{fig:recon_fig}
\end{figure}

}

\section{Deleted Cluster Reconstruction} \label{sec:cluster}
The reconstruction attack of Section \ref{sec:Singleton} focused on recovering the only deleted instance from the training set. In this section we generalize the experiments of Section \ref{sec:Singleton} to where the data in the data set $\cS$ comes from \emph{multiple sources} each sampled from a different ``cluster''. Then, the data from one cluster is removed, and the adversary's goal is to find the description of the cluster whose data is removed. More specifically, each cluster's instances will be sampled from a well defined distribution described by a binary vector ``center'' in $\bits^d$, and the goal of the adversary is to find this particular vector. The memorization effect of highly-accurate models on clustered data was also studied in the work of \cite{brown2021memorization}, and our work experimentally show the power of \emph{deletion reconstruction attacks} in this setting as well. We start by describing the security game.


As part of the setting, before defining the security game we first define the clustering distribution. In this experiment we define $\cX$ as the set of all $d$-dimensional strings $\{0, 1\}^d$ and $\cY = [\ell]$. Furthermore, for each class $c \in [\ell]$, there is a cluster center $x_c = b_1\dots b_d$ randomly drawn from the uniform distribution over $\{0, 1\}^d$. Now we define a clustering distribution $S_n$ as $n$ independent examples $(x_1, y_1), \dots (x_n, y_n)$, that for each $i \in [n]$, $y_i$ is uniformly sampled from $[\ell]$, and $x_i \gets \textbf{BSC}_p(x_{y_i})$,   where $\textbf{BSC}$ stands for binary symmetric channel, which flips every character $x_i$ in $x_c$ with a crossover probability $p$ for every $i \in [d]$. Then we define the deleted clustering reconstruction security based on Definition \ref{def:Del-Recon}.

\begin{definition}[Deleted cluster reconstruction] \label{def:Del-Clu-Recon}
This definition is similar to Definition \ref{def:Del-Recon} with the following differences.
%Let $\Learn$ be a learning algorithm, $\Del$ be a deletion mechanism for $\Learn$, and 
(1) $S_n$ is the clustering distribution defined above. (2) In the ``Deletion'' step, a random $y \gets \cY$  is selected and all $(x,y) \in \cS$ are deleted. Success is measured  based on the center of the cluster $y$.
\remove{
%Consider the following game played between the adversary $\Adv$ and challenger $\Chal$.
\begin{enumerate}
    \item {\bf Sampling the data and random selection.} $\Chal$ picks a data set $\{e_1 \dots e_n\} = \cS \gets S_n$ of size $n$. 
    % by choosing $n$ i.i.d samples $e_0,\dots,e_n \gets D$. 
    It also chooses $c \gets \cY$ at random. %The challenger   picks $i\neq j$ at random and sends $(e_i,e_j)$ (but not the rest of $\cS$) to $\Adv$. 
        \item   {\bf Oracle access  before deletion.}  The challenger $\Chal$   trains $\model \gets \Learn(\cS)$.
  The adversary $\Adv$ is then given \emph{oracle} access to $\model$. At the end of this step, the adversary instructs moving to the next step.
  
      \item {\bf Deletion.} The challenger obtains $\model_{-c} \gets \Del(h,\cS_c)$, where $\cS_c = \{(x, y) \in \cS \mid y = c \}$.%   and if $b=1$, then $\model_\del \gets \Del(h,e_j)$.
     \item {\bf Oracle access after deletion.}     
        The adversary $\Adv$ (who cannot access   $\model$ anymore) is given \emph{oracle} access to  $\model_{-c}$.
    
    \item {\bf Adversary's guess and the output.}  The adversary outputs $x'_c$. 
\end{enumerate}
 For a similarity metric  $\dis$ defined on $\cX$, the adversary $\Adv$ is called a  \emph{$(\rho,\eps)$-successful deletion reconstruction} attack  if it holds that $\Pr[\dis(x'_c, x_c) \leq \eps ]\geq \rho$. 
%  When  $\Pr[e \neq e_i  ]\geq \rho$, we simply call $\Adv$ $\rho$-successful. 
For bounded $\dis(\cdot,\cdot) \in [0,1]$ and an adversary $\Adv$, we define the  \emph{expected accuracy} of $\Adv$ as $1-\Ex[\dis(x'_c, x_c)]$.
}
\end{definition}


% On this experiment, we design the following adversary.

% \begin{alg}[Attack $\DelCluRecon$]  \label{alg:clu_recon}
% % The attack is defined with a combination function $\textbf{Combine}$, which gives an prediction from a subset of examples. 
% Suppose the adversary is given oracle access to $\model$ and $\modelDel$, along with a set of instances $\cS$, $\cS \gets \cX^m$. The attack then proceeds as follows:
% \begin{itemize}
%     \item For all $x \in \cS$, query model $\model$ and $\modelDel$. 
%     \item Create the subset $\cS' \subseteq \cS$ where $\cS' = \left\{ x \mid \model(x) \neq \modelDel(x), x \in \cS \right\}$.
%     % \item Return $x' = \textbf{Combine}(\cS')$.
%     \item Return $x = b'_1 \dots b'_d$, where $\forall i \in [d]$,
%     $$b'_i = \argmax_{b \in \{0, 1\}} \sum_{b_1 \dots b_d \in \cS'} \mathbf{1}\{b_i = b\}.$$\qedhere
% \end{itemize}
% \end{alg}


% \Mnote{many of my comments above apply to this subsection as well. also pleas make the format look like the stuff in Section 3. Please put parenthesis around bit vectors and update the experiment picture. Also, we need to include a security game for the cluster deletion reconstruction, based on how the experiments are actually done!} 

\noindent{\bf Experiment details.} This experiment follows the game of Definition \ref{def:Del-Clu-Recon}. The learning algorithm $\Learn$ is the $1$-nearest neighbor: for every string $x$ in the space $\{0, 1\}^d$, the learning algorithm returns the label of its nearest example in the training dataset.  Furthermore, we use \emph{the  same adversary} of Algorithm \ref{alg:recon_general} to reconstruct the instance.
% \end{itemize}
% for an integer $n$ and  The training dataset is then generated by first uniformly sample a class label $y \in [n]$, and then sample an example $x = \textbf{BSC}_p(x_c)$, where $\textbf{BSC}$ stands for binary symmetric channel, which flips every character $x_i$ in $x_c$ with a crossover probability $p$ for every $i \in [d]$. Let $l$ be the examples in the training dataset.
 % In this experiment, we assume all the examples from cluster $c$ is removed in this case. Adversary in this experiment then guesses the cluster center $x_c$ by first randomly sampling $m$ examples uniformly from $\{0, 1\}^d$. The adversary queries these $m$ examples to both models, and denote every examples that has prediction label changed. Suppose there are $m'$ such examples whose prediction label has changed. Then adversary guesses $x' = b'_1 \dots b'_d$, where $b'_i = \argmax_{b \in \{0, 1\}} \sum_{j = 1}^{m'} \mathbf{1}\{b^{(j)}_i = b\}$ is a majority vote on the $m'$ examples. 
%
In the experiment, we let $d = 100$, $l = |\cY|=100$, $n=1000$, and $m = 2000$. We then varies the crossover probability $p$ in the generation process. Similar to the experiment

% Similar to the last experiment, we measure two metrics, \textit{Approximated Accuracy} and \textit{Average correct indices}, to study the performance of the reconstruction adversary.

\paragraph{Results.} 
We show the experiment results in Figure \ref{fig:recon_cluster}. This result show that while the cluster center is hidden and not directly included in the deleted examples, our adversary can still successfully reconstruct the center of the cluster with high probability.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{Figures/exp2.pdf}
    \caption{Y-axis is Adversary's performance and X-axis is crossover probability. The blue curve shows the largest $\rho$ where the attack is a $(\rho, 1 -\rho)$-successful cluster reconstruction attack  and the orange curve shows the expected accuracy.}
    \label{fig:recon_cluster}
\end{figure}


==> MoreExpNew.tex <==
{\color{blue}{}
\section{Deletion Inference with the Reference Example Outside Training Dataset} \label{sec:outside_training}

The security game in Definition \ref{def:WeakDelPriv} specifically requires both examples in the training set. We extend the setting in this section by letting one of the example outside the training dataset.

\begin{definition}[Variation of Deletion inference that example outside the training dataset] \label{def:WeakDelPrivOut}
Let $\Learn$ be a learner and $\Del$ be a deletion mechanism for $\Learn$. For distribution $S_n$  on data sets of size $n$, consider the following game   between the adversary $\Adv$ and challenger $\Chal$.
\begin{enumerate}
    \item {\bf Sampling the data and revealing the challenges.} $\Chal$ picks a data set $\set{e_1,\dots,e_n}=\cS \gets S_n$ of size $n$. The challenger   picks $i\neq j \in [n]$ at random and sends $(e_i,e_j)$  to $\Adv$ (but not the rest of $\cS$). 
        \item {\bf Oracle access  before deletion.}  The challenger tosses a coin $b \gets \bits$ at random and does as follows. If $b=0$, then we let $\cS' \gets \cS - e_j$,   and if $b=1$, then we let $\cS' \gets \cS - e_i$. The challenger $\Chal$ then trains $\model \gets \Learn(\cS')$.
  The adversary $\Adv$ is then given \emph{oracle} access to $\model$. At the end of this step, the adversary instructs moving to the next step.
  
      \item {\bf Deletion.} If $b=0$, then $\model_\del \gets \Del(h,e_i)$,   and if $b=1$, then $\model_\del \gets \Del(h,e_j)$.
     \item {\bf Oracle access after deletion.}     
        The adversary $\Adv$ (who cannot access   $\model$ anymore) is given {oracle} access to  $\model_\del$.
    
    \item {\bf Adversary's guess and the output.}  The adversary  sends bit  $b'$ to the challenger, and it wins if $b'=b$.
\end{enumerate}

The scheme $(\Learn,\Del)$ is called \emph{$\rho$  insecure  against deletion inference} for data distribution $S_n$, if there is a PPT adversary $\Adv$ whose success probability in the game above is at least $\rho$.  (Note that achieving $\rho=1/2$ is trivial.) 

Similar to deletion inference in Definition \ref{def:WeakDelPriv}, we can then define instance reveal deletion inference and label deletion inference for the case when the reference example is outside the dataset.
% Consider a modified  game, in which the adversary is  given \emph{only} the instances $(x_i,x_j)$ where $e_i=(x_i,y_i),e_j=(x_j,y_j)$ (rather than full labeled examples $(e_i,e_j)$). We call this game the \emph{instance  (revealed)} deletion inference. If an adversary has success probability   at least   $\rho$  in the instance deletion inference game, then the scheme $(\Learn,\Del)$ is called $\rho$  insecure  against \emph{instance} deletion inference for distribution $S_n$. Similarly, we define \emph{label} deletion inference, where only the label $(y_i,y_j)$ are revealed to the adversary, and $\rho$-insecurity against such attacks accordingly.
\end{definition}

The major difference between Definition \ref{def:WeakDelPrivOut} and Definition  \ref{def:WeakDelPriv} is that the model  $\model$ before deletion does not include one of the two challenge examples into the training dataset. This example is not included in neither models.

\paragraph{Our deletion inference attacks.} 

Interestingly, for the security game in Definition \ref{def:WeakDelPrivOut}, Algorithm \ref{const:delinflbl} and Algorithm \ref{const:delinf} can still be applied. It is because the loss of an example never in the training dataset should remain similar.

\paragraph{Experiment Details.} We perform the exact same experiment following Section \ref{sec:del_inf_regression} and Section \ref{sec:del_inf_classification}. The only difference is we follow the security game in Definition \ref{def:WeakDelPrivOut} instead, i.e., one example is left outside the dataset.

\paragraph{Results.}
The result of the experiments are shown in Table \ref{tab:deletion_reg_outside} and Table \ref{tab:deletion_class_outside} for regression and classification models respectively.
\begin{table*}[ht]
\begin{tabular}{l|ll|ll}
\hline 
                    & \multicolumn{2}{c|}{Boston Housing} & \multicolumn{2}{c}{Diabetes} \\ \hline
                    \textit{Learning Method} & $\DInfWith$  & $\DInfNo$ & $\DInfWith$  & $\DInfNo$  \\ \hline
Linear regression & 97.10\%  & 95.70\%  & 99.50\%  & 99.20\%  \\ \hline
SVM               & 96.40\%  & 91.80\%  & 99.20\%  & 100.00\% \\ \hline
Lasso regression  & 96.70\%  & 94.00\%  & 98.90\%  & 97.10\%  \\ \hline
Decision tree     & 90.40\% & 73.90\% & 94.30\% & 83.70\% \\ \hline
\end{tabular}
\caption{Success probabilities of Definition~\ref{def:WeakDelPrivOut} for the attacks on regressors and different data sets.}
\label{tab:deletion_reg_outside}
\end{table*}

\begin{table*}[ht]
\begin{tabular}{l|ll|ll|ll}
\hline 
                    & \multicolumn{2}{c|}{Iris} & \multicolumn{2}{c}{Wine} & \multicolumn{2}{|c}{Breast Cancer} \\ \hline
                    \textit{Learning Method} & $\DInfWith$  & $\DInfNo$ & $\DInfWith$  & $\DInfNo$ & $\DInfWith$      & $\DInfNo$      \\ \hline
Logistic Regression & 88.70\%      & 87.00\%   & 79.00\%      & 71.80\%   & 64.40\%          & 56.20\%        \\ \hline
Decision Tree       & 95.20\%     & 98.00\%  & 87.90\%     & 98.60\%  & 93.20\%         & 98.10\%       \\ \hline
SVM                 & 67.30\%      & 55.60\%   & 76.90\%      & 67.10\%   & 74.10\%          & 55.80\%  \\ \hline
Random Forest       & 86.30\%      & 80.00\%   & 76.70\%      & 58.30\%   & 86.50\%          & 72.80\%   \\ \hline
\end{tabular}
\caption{Success probabilities of Definition~\ref{def:WeakDelPrivOut} for the attacks on classifiers and different data sets.}
\label{tab:deletion_class_outside}
\end{table*}

The performance is slightly worse than the security game of Definition \ref{def:WeakDelPriv}, however, the success probability is still high in many settings.

\section{Study the privacy under deletion inference with synthesized dataset}

In this section, we further study the privacy under deletion inference with synthesized dataset. Generally the experiment follows from the experiments in Section \ref{sec:del_inf_regression} and Section \ref{sec:del_inf_classification}, but we use synthesized datasets instead. Synthesized datasets give us more control, including how specific property impacts the privacy of the model.


\subsection{Regressors on Synthesized Dataset}
We start by showing deletion inference can succeed on synthesized dataset. We follow the experiments in Section \ref{sec:del_inf_regression}. Specifically, we follow the security game described in Definition \ref{def:WeakDelPriv} and Definition \ref{def:WeakDelPrivOut}.

\paragraph{Experiment details.}
We now describe how we generate the synthesized dataset. For an example $e_i = (x_i, y_i)$, we assume the instance $x_i$ is drawn from a $d$-dimensional Gaussian distribution $N(\mathbf{0},\bfI)$ where $\mathbf{0}=(0,\dots,0),\mathbf{1}=(1,\dots,1)$ and $\bfI$ is the identity matrix. We further assume label $y_i = \angles{\bfw,x_i} + \mathbf{\eps}_i$ follows a linear ground-truth function with fixed $\bfw$ and an independent additive Gaussian noise from $\mathbf{\eps} \sim N(\mathbf{0}, r \cdot \bfI)$ represented by $\mathbf{\eps}$. We draw $n$ random samples from the data distribution to create a training dataset. 

$d$ stands for the dimension, $r$ stands for the noise size, and $n$ stands for the training dataset size are the three hyperparameters in the experiment that we will discuss.

We use Algorithm \ref{const:delinflbl} and Algorithm \ref{const:delinf} for the adversary.

\subsubsection{Basic result.} We start by letting $d = 10$, $r = 0.1$ and $n = 1000$. We run the experiment with different learning algorithms including linear regression, Lasso regression, SVM, and decision tree. 
The result is shown in Table \ref{tab:deletion_reg_syn}.

\begin{table*}[ht]
\begin{tabular}{l|ll|ll}
\hline 
                    & \multicolumn{2}{c|}{Inside $\cS$} & \multicolumn{2}{c}{Outside $\cS$} \\ \hline
                    \textit{Learning Method} & $\DInfWith$  & $\DInfNo$ & $\DInfWith$  & $\DInfNo$  \\ \hline
Linear regression & 99.60\%  & 99.30\%  & 99.50\%  & 98.70\%  \\ \hline
SVM               & 91.20\%  & 89.70\%  & 90.50\%  & 89.40\% \\ \hline
Lasso regression  & 99.80\%  & 93.90\%  & 99.80\%  & 92.80\%  \\ \hline
Decision tree     & 100.00\% & 100.00\% & 92.90\% & 82.80\% \\ \hline
\end{tabular}
\caption{Success probabilities for the attacks on regressors and synthesized data sets, where ``Inside $\cS$'' stands for the security game of Definition \ref{def:WeakDelPriv} and ``Outside $\cS$'' stands for the security game of Definition \ref{def:WeakDelPrivOut}.}
\label{tab:deletion_reg_syn}
\end{table*}

The result show that our simple deletion inference adversary can achieve close to $100\%$ success probability with the synthetic dataset.

\subsubsection{Varying training dataset size $n$}
We now study that how the size of the training dataset $n$ impacts the adversary's success probability. We let $n = 1000, 5000, 10000, 50000$ and then study the success probability of the adversary $\ref{const:delinflbl}$ on the linear regression model. The result is included in the figure \ref{fig:trend_syn_n}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/trend_syn_n.pdf}
    \caption{How different size of training dataset $n$ impacts the success probability, where ``Inside $\cS$'' stands for the security game of Definition \ref{def:WeakDelPriv} and ``Outside $\cS$'' stands for the security game of Definition \ref{def:WeakDelPrivOut}.}
    \label{fig:trend_syn_n}
\end{figure}

The result show that when $n$ increases, the success probability of the adversary generally goes down. However, even if $n=50000$, the success probability is still $96\%$ in this simple case, indicating even large dataset is potentially vulnerable to the deletion inference adversary.

\subsubsection{Varying dimension $d$}
We then study that how the dimension $d$ impacts the adversary's success probability. We let $d = 10, 50, 100, 500$ and then study the success probability of the adversary $\ref{const:delinflbl}$ on the linear regression model. The result is included in the figure \ref{fig:trend_syn_dim}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/trend_syn_dim.pdf}
    \caption{How different dimension $d$ of the synthesized dataset impacts the success probability, where ``Inside $\cS$'' stands for the security game of Definition \ref{def:WeakDelPriv} and ``Outside $\cS$'' stands for the security game of Definition \ref{def:WeakDelPrivOut}.}
    \label{fig:trend_syn_dim}
\end{figure}

The result show that when $d$ increases, the success probability of the adversary generally goes up. A possible explanation is that because learning becomes harder when $d$ increases, and it also requires the model to memorize more of the training dataset.

\subsubsection{Varying noise level $r$}
We then study that how the noise level $r$ impacts the adversary's success probability. We let $r = 0.01, 0.1, 1, 10$ and then study the success probability of the adversary $\ref{const:delinflbl}$ on the linear regression model. The result is included in the figure \ref{fig:trend_syn_r}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/trend_syn_r.pdf}
    \caption{How different noise level $r$ of the synthesized dataset impacts the success probability, where ``Inside $\cS$'' stands for the security game of Definition \ref{def:WeakDelPriv} and ``Outside $\cS$'' stands for the security game of Definition \ref{def:WeakDelPrivOut}.}
    \label{fig:trend_syn_r}
\end{figure}

The result show that when $r$ increases, the success probability of the adversary generally goes up. Similar to the dimension, A possible explanation is that because learning becomes harder when noise level $r$ increases, and it also requires the model to memorize more of the training dataset.


\section{Reducing two example deletion inference into one example}
\label{sec:reduce_1challenge}

 Definition \ref{def:WeakDelPriv} includes two challenger examples and asking an adversary to find out which one is the actual subject of attack. One may argue such setting is redundant, that only using one challenge is enough to test the adversary's capability. We include some discussions about this topic in this section.
 
 In fact, the setting is a standard framework in cryptography (e.g., this is how CPA/CCA security is defined), and is also implicitly used in the definition of differential privacy where indistinguishability is the key. The attack follows Definition \ref{def:WeakDelPriv} is a “weak” attack in the sense that “real world” attacks (e.g., as modeled in crypto definitions such as CPA or CCA security) might deal with adversaries who in some way have picked their targets, and we will show that even weak attacks can succeed.

Interestingly, the two challenge setting can be related to settings where only one challenge exists and the adversary wants to find the solution through a hybrid argument. Namely, suppose you have an adversary who breaks the “2 challenge” game and you are given “1 challenge” only. The reduction, basically, attaches a new challenge (whose answer is known to the reduction) to the given challenge, and then runs the “2 challenge” adversary as a black-box. How to exactly pick this extra challenge and the analysis are  not totally trivial, but once done properly it is also not hard to show that: if the “2 challenge” attacker wins with probability close to 1 (which is the case in our case), so does the “1 challenge” adversary. The limitation is that such reductions only work if the adversary has access to a good source of “extra challenge” to sample from, but that is at least not an issue when the attack is “information theoretic” (e.g., as in differential privacy). 

Furthermore, we can simply reduce our attacks to  the “1 challenge” case as well, because all our attacker does is to compare the “change in the loss”, and hence one can use a predefined “threshold” (applied to the change in the loss) to judge whether a given challenge is deleted or not. Using this trick, one can indeed adapt our attacks to the “1 challenge” case as well.

}



==> macros.tex <==
%\newcommand{\ifcompact}{\iftrue}
%\ifcompact
%\newcommand{\paragraph}[1]{\medskip \noindent {\bf #1}}
%\fi

%\newcommand{\DataApp}{\mathsf{Data}\text{-}\mathsf{App}}
\newcommand{\DInfWith}{\mathsf{Del}\text{-}\mathsf{Inf}\text{-}\mathsf{Exm}}
\newcommand{\DInfNo}{\mathsf{Del}\text{-}\mathsf{Inf}\text{-}\mathsf{Ins}}
\newcommand{\DelRecon}{\mathsf{Del}\text{-}\mathsf{Ins}\text{-}\mathsf{Rec}}
\newcommand{\DelCluRecon}{\mathsf{Del}\text{-}\mathsf{Clu}\text{-}\mathsf{Rec}}
\newcommand{\LabelApp}{\mathsf{Ins}\text{-}\mathsf{Rev}\text{-}\mathsf{Lbl}\text{-}\mathsf{Rec}}
\newcommand{\LabelInf}{\mathsf{Del}\text{-}\mathsf{Lbl}\text{-}\mathsf{Rec}}
\usepackage{centernot}
\newcommand{\Score}{\mathsf{Score}}
\newcommand{\Learn}{\mathsf{Learn}}
\newcommand{\ERM}{\mathsf{ERM}}

\newcommand{\Add}{\mathsf{Add}}
\newcommand{\Del}{\mathsf{Del}}
\newcommand{\Eval}{\mathsf{Eval}}

\newcommand{\DataCol}{\mathsf{DatCol}}
\newcommand{\DelReq}{\mathsf{DelReq}}
\newcommand{\Env}{\mathsf{Env}}
\newcommand{\Records}{\mathcal{U}}
\newcommand{\Otilde}{\wt{O}}
\newcommand{\Leak}{\mathsf{leak}}
\newcommand{\Alg}{\mathsf{Alg}}

\newcommand{\metric}{{{\mathsf{d}}}}
\newcommand{\metr}{\metric}
\newcommand{\Ball}{\mathcal{B}all}
\newcommand{\Sph}{\mathcal{S}phr}

\newcommand{\diam}{\mathsf{Diam}}
\newcommand{\Levy}{Lévy\xspace}
\newcommand{\Lovasz}{Lovász\xspace}
\newcommand{\real}{\mathsf{real}}
\newcommand{\ideal}{\mathsf{ideal}}

\newcommand{\paragcompact}[1]{\noindent{\bf #1}}

\newcommand{\paragdot}[1]{\paragraph{#1.}}
%\newcommand{\Y}{\ensuremath{\mathcal{Y}}\xspace} % X
%\newcommand{\X}{\ensuremath{\mathcal{X}}\xspace} % X

\newcommand{\HD}{\mathsf{HD}}

\newcommand{\con}{{\bm \upalpha}}
\newcommand{\msr}{{\bm{\upmu}}}

\newcommand{\RemInLab}{\mathsf{RemInLab}}
\newcommand{\mal}{\wt}

\newcommand{\error}{\mathsf{Err}}
\newcommand{\Error}{\error}

\newcommand{\alphaDist}{{\bm \upalpha}}
\newcommand{\Risk}{\mathsf{Risk}}
\newcommand{\Rob}{\mathsf{Rob}}



\newcommand{\Tam}{\mathsf{Tam}}
\newcommand{\TamAb}{\mathsf{TamAb}}
\newcommand{\AppTam}{\mathsf{AppTam}}
\newcommand{\AppTamAb}{\mathsf{AppTamAb}}
%\newcommand{\ORTam}{\mathsf{ORSam}}
%\newcommand{\KRTam}{\mathsf{KRSam}}
\newcommand{\Inv}{\mathsf{Inv}}
\newcommand{\Ideal}{\mathsf{Ideal}}
\newcommand{\Trans}{\mathsf{Trans}}
% \newcommand{\Small}{\mathsf{Small}}
\newcommand{\UnBal}{\mathsf{UnBal}}
\newcommand{\Good}{\mathsf{Good}}
\newcommand{\High}{\mathrm{High}}
\newcommand{\Low}{\mathrm{Low}}
\newcommand{\BigOut}{\mathrm{Big}}
\newcommand{\SmallOut}{\mathrm{Small}}


\newcommand{\xDist}{\mathbf{x}}
\newcommand{\yDist}{\mathbf{y}}
\newcommand{\zDist}{\mathbf{z}}
\newcommand{\tDist}{\mathbf{t}}
\newcommand{\TDist}{\mathbf{T}}
\newcommand{\WDist}{\mathbf{W}}
\newcommand{\sDist}{\mathbf{s}}
\newcommand{\uDist}{\mathbf{u}}
\newcommand{\vDist}{\mathbf{v}}
\newcommand{\wDist}{\mathbf{w}}



\newcommand{\XDist}{\mathbf{X}}
\newcommand{\UDist}{\mathbf{U}}
\newcommand{\trainDist}{\UDist}

\newcommand{\xDistVec}{\ol{\xDist}}
\newcommand{\yDistVec}{\ol{\yDist}}
\newcommand{\zDistVec}{\ol{\zDist}}
\newcommand{\tDistVec}{\ol{\tDist}}
\newcommand{\sDistVec}{\ol{\sDist}}
\newcommand{\uDistVec}{\ol{\uDist}}
\newcommand{\vDistVec}{\ol{\vDist}}
\newcommand{\wDistVec}{\ol{\wDist}}


\newcommand{\insDist}{\xDist}
\newcommand{\instDist}{\insDist}

\newcommand{\xVec}{\ol{x}}
\newcommand{\yVec}{\ol{y}}
\newcommand{\zVec}{\ol{z}}
\newcommand{\tVec}{\ol{t}}
\newcommand{\sVec}{\ol{s}}
\newcommand{\uVec}{\ol{u}}
\newcommand{\vVec}{\ol{v}}
\newcommand{\wVec}{\ol{w}}

\newcommand{\alVec}{{\ol{\alpha}}}
\newcommand{\alK}{{\bfK_\alVec}}
\newcommand{\alk}{{\bfK_\alVec}}
\newcommand{\alHD}{\HD_{\alVec}}

\newcommand{\SDist}{\mathbf{S}}

\newcommand{\uRP}{{\wt{\uDist}}}

\renewcommand{\th}{^\mathrm{th}}
\newcommand{\jointSamp}[2]{\langle #1 \,\, \| \, {#2}\rangle}
\newcommand{\fvers}{(Please see the full version for the proof.) }

\newcommand{\overbar}[1]{\mkern 1.9mu\overline{\mkern-2.9mu#1\mkern-0.5mu}\mkern 1.9mu}
\newcommand{\overbarr}[1]{\mkern 1.9mu\overline{\mkern-0.9mu#1\mkern-3.5mu}\mkern 1.9mu}
%\newcommand{\X}{\overbar{X}}
%\newcommand{\Y}{\overline{Y}}
%\newcommand{\Yd}{\overbarr{Y_\delta}}
%\newcommand{\Z}{\overbar{Z}}

%\renewcommand{\R}{\olverline{R}}
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newcommand{\spn}{\mathrm{Span}}
\newcommand{\EQref}[1]{Equation~(\ref{#1})}
\newcommand{\VP}{\mathrm{ValPrf}}
\newcommand{\EX}{\mathsf{Ext}}
\newcommand{\Dn}{D^{\scriptscriptstyle (n)}}

\newcommand{\cost}{\mathsf{cost}}
\newcommand{\avgcost}{\overline{\cost}}


\newcommand{\KLsimp}{D_\mathsf{\scriptscriptstyle KL}}
\newcommand{\KL}[2]{D_\mathsf{\scriptscriptstyle KL}(#1||#2)}
\newcommand{\KLn}[2]{D^{\scriptscriptstyle (n)}_\mathsf{\scriptscriptstyle KL}(#1||#2)}

\newcommand{\MDsimp}{D_{\scriptscriptstyle \infty}}
\newcommand{\MD}[2]{D_{\scriptscriptstyle \infty}(#1||#2)}
\newcommand{\MDn}[2]{D^{\scriptscriptstyle (n)}_{\scriptscriptstyle\infty}(#1||#2)}

\newcommand{\SDsimp}{D_\mathsf{\scriptscriptstyle SD}}
\newcommand{\SD}{\Delta}%[2]{D_\mathsf{\scriptscriptstyle SD}(#1,#2)}
\newcommand{\SDn}[2]{D^{\scriptscriptstyle (n)}_\mathsf{\scriptscriptstyle SD}(#1,#2)}

\newcommand{\minE}[1]{\mathrm{H}_{\scriptscriptstyle \infty}(#1)}

\newcommand{\pfix}[2]{ {#1}_{\leq #2}}
\newcommand{\pofix}[2]{#1_{\geq #2 }}
\newcommand{\dmax}{\mathsf{max}_\delta}
%\newcommand{\avr}[2]{\Ex[#1(#2)]}
\newcommand{\dMax}{\mathsf{Max}_{\geq \delta}}
\newcommand{\dlMax}{\mathsf{Max}_{< \delta}}

\newcommand{\Exists}{\exists\,}
\newcommand{\Forall}{\forall\,}
\newcommand{\fDist}{\mathbf{f}}
\newcommand{\aSF}{\mathsf{a}}
\newcommand{\gSF}{\mathsf{g}}
\newcommand{\hSF}{\mathsf{h}}

\newcommand{\avr}[2]{\ifthenelse{\equal{#2}{}}{\aSF({#1})}{\ifthenelse{\equal{#2}{0}}{\aSF(\emptyset)}{\aSF({#1}_{\leq #2})}}}

\newcommand{\avrMax}[2]{\ifthenelse{\equal{#2}{}}{\aSF^*({#1})}{\ifthenelse{\equal{#2}{0}}{\aSF^*(\emptyset)}{\aSF^*({#1}_{\leq #2})}}}

\newcommand{\avrApp}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\aSF}({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{\aSF}(\emptyset)}{\tilde{\aSF}({#1}_{\leq #2})}}}

\newcommand{\avrAppMax}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\aSF}^*({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{\aSF}^*(\emptyset)}{\tilde{\aSF}^*({#1}_{\leq #2})}}}

\newcommand{\ArgMax}[2]{\ifthenelse{\equal{#2}{}}{\hSF({#1})}{\ifthenelse{\equal{#2}{0}}{\hSF(\emptyset)}{\hSF({#1}_{\leq #2})}}}

\newcommand{\AppArgMax}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\hSF}({#1})}{\ifthenelse{\equal{#2}{0}}{\tilde{\hSF}(\emptyset)}{\tilde{\hSF}({#1}_{\leq #2})}}}

\newcommand{\Err}{\mathcal{E}}
\newcommand{\expectedsub}[2]{\ensuremath{\mathop{{}\mathbf{E}}_{#1}\left[#2\right]}\xspace}
\newcommand{\charac}{\mathbf{1}}


\newcommand{\gain}[2]{\ifthenelse{\equal{#2}{}}{\gSF(#1)}{\gSF(#1_{\leq #2})}}
\newcommand{\gainMax}[2]{\ifthenelse{\equal{#2}{}}{\gSF^*(#1)}{\gSF^*(#1_{\leq #2})}}
\newcommand{\gainApp}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\gSF}(#1)}{\tilde{\gSF}(#1_{\leq #2})}}
\newcommand{\gainAppMax}[2]{\ifthenelse{\equal{#2}{}}{\tilde{\gSF}^*(#1)}{\tilde{\gSF}^*(#1_{\leq #2})}}

%\newcommand{\avGain}(3]{{\mathcal{G}}_{#3}(#1_{\leq #2 -1}]}
%\newcommand{\avAbGain}(3]{\mathcal{A}_{#3}(#1_{\leq #2 -1}]}
%\newcommand{\avSqGain}(3]{\mathcal{Q}_{#3}(#1_{\leq #2 -1}]}



\newcommand{\RTam}{\mathsf{RejSam}}
\newcommand{\RTamk}{\mathsf{RejSam}_{k}}
%\newcommand{\RTamd}{\mathsf{RSam}_\delta}


\newcommand{\var}[2]{\Var[#1(#2)]}

% \newcommand{\pr}[2][]{\Pr_{\ifthenelse{\isempty{#1}}{}{{#1}}}\left[{#2}\right]}
% Replacing the \pr command for now because I don't understand how to use the above.
\newcommand{\pr}[1]{\Pr\left[{#1}\right]}
\newcommand{\prob}[2]{\Pr_{{#1}}\left[{#2}\right]}

\newcommand{\GTam}{\mathsf{GTam}}
\newcommand{\EGTam}{\mathsf{EGTam}}

\newcommand{\LimSup}{\operatorname{limSup}}
%\newcommand{\sup}{\operatorname{sup}}
\newcommand{\pmbits}{\{+1,-1\}}
\newcommand{\pmint}{[-1,+1]}
%\newcommand{\Tam}{\Tam}
\newcommand{\IdealTam}{\mathsf{IdTam}}
\newcommand{\EffTam}{\mathsf{EffTam}}



\newcommand{\dis}{\mathsf{dis}}
% Oracle subroutines
\newcommand{\distO}{\mathbf{O}}
\newcommand{\setup}{\mathsf{G}}
\newcommand{\findsk}{{\mathsf{G}^{-1}}}
\newcommand{\enc}{\operatorname{Enc}}
\newcommand{\dec}{\operatorname{Dec}}
\newcommand{\rev}{\mathsf{rev}}
\newcommand{\decFull}{\operatorname{DecFull}}
\newcommand{\eval}{\mathsf{eval}}
\newcommand{\gi}{\mathsf{gi}}
\newcommand{\gc}{\mathsf{gc}}

\newcommand{\kgen}{\mathsf{K}}
\newcommand{\test}{\mathsf{T}}
\newcommand{\testatt}{mathsf{T}}
\newcommand{\V}{\mathsf{V}}
\newcommand{\Pred}{\mathsf{P}}
\newcommand{\Func}{\mathsf{F}}

% Garbling and RE
\newcommand{\lbl}{\mathsf{label}}
\newcommand{\GCircuit}{\mathsf{Garb}}
\newcommand{\GInput}{\mathsf{GInput}}
\newcommand{\GEval}{\mathsf{Eval}}
\newcommand{\Circuit}{\mathsf{C}}
\newcommand{\hCircuit}{\hat{\mathsf{C}}}
\newcommand{\hFun}{\hat{\mathsf{F}}}
\newcommand{\Fun}{\mathsf{F}}
\newcommand{\GarbledCircuit}{\widetilde{\Circuit}}
\newcommand{\wire}{w}
\newcommand{\inp}{\mathsf{inp}}
\newcommand{\inpsize}{\mathsf{inpsize}}
\newcommand{\out}{\mathsf{out}}
\newcommand{\CircSim}{\mathsf{CircSim}}
\newcommand{\Garbled}[1]{\widetilde{#1}}
\newcommand{\Output}{y}
\newcommand{\Input}{x}
\newcommand{\GarbledInput}{\widetilde x}
\newcommand{\InputKey}{s^{\mathsf{in}}}
\newcommand{\InputSize}{m}
\def\indc{\stackrel{{\tiny{\mathrm{comp}}}}{\approx}}
\newcommand{\RE}{\mathsf{RE}}
\newcommand{\REenc}{\mathsf{RE.enc}}
\newcommand{\REdec}{\mathsf{RE.dec}}

\newcommand{\HandleEval}{\mathtt{HandleEval}}
\newcommand{\ConstructHelpers}{\mathtt{ConstHelp}}
\newcommand{\Reduct}{\mathtt{SecurityRed}}
\newcommand{\Reduc}{\Reduct}

% Algorithms
\newcommand{\scheme}{\mathcal{E}}
\newcommand{\newScheme}{\dot{\scheme}}
\newcommand{\newSchemex}{\ddot{\scheme}}
\newcommand{\newG}{\dot{G}}
\newcommand{\newE}{\dot{E}}
\newcommand{\newD}{\dot{D}}
\newcommand{\newpk}{\dot{pk}}
\newcommand{\newsk}{\dot{sk}}
\newcommand{\newc}{\dot{c}}
\newcommand{\newGx}{\ddot{G}}
\newcommand{\newEx}{\ddot{E}}
\newcommand{\newDx}{\ddot{D}}
\newcommand{\newpkx}{\ddot{pk}}
\newcommand{\newskx}{\ddot{sk}}
\newcommand{\newcx}{\ddot{c}}
\newcommand{\newp}{\dot{p}}
\newcommand{\newpx}{\ddot{p}}
\newcommand{\newq}{\dot{q}}
\newcommand{\newqx}{\ddot{q}}


% Events Notation
\newcommand{\Bad}{\mathrm{Bad}}
\newcommand{\Miss}{\mathrm{Miss}}
\newcommand{\Hit}{\mathrm{Hit}}
\newcommand{\Disjoint}{\mathrm{Disjoint}}

% Query Set Notation
\newcommand{\sets}[1]{\mathsf{#1}}
\newcommand{\Q}[2]{(#2 \xrightarrow[#1]{} \; ?)}
\newcommand{\QA}[3]{(#2 \xrightarrow[#1]{} #3)}
\newcommand{\OrigG}{\sets{OrigG}}
\newcommand{\OrigE}{\sets{OrigE}}
\newcommand{\OrigD}{\sets{OrigD}}
\newcommand{\LearnG}{\sets{LearnG}}
\newcommand{\LocalE}{\sets{LocalE}}
\newcommand{\AllE}{\sets{AllE}}
\newcommand{\LocalD}{\sets{LocalD}}
\newcommand{\EvalD}{\sets{EvalD}}
\newcommand{\SO}{S}
\newcommand{\HintGEnc}{\sets{H}}
\newcommand{\HintGEnci}[1]{\sets{H}^{#1}_{\newE}}
\newcommand{\HintEDec}{\sets{H}}
\newcommand{\HintEDeci}[1]{\sets{H}^{#1}_{\newDx}}
\newcommand{\HintGEncSim}{\HintGEnc^*}
\newcommand{\HintEDecSim}{\HintEDec^*}
\newcommand{\OrigESim}{\sets{\OrigE^*}}
\newcommand{\LocalESim}{\sets{\LocalE^*}}
\newcommand{\LearnGSim}{\LearnG}
\newcommand{\EvalDSim}{\EvalD^*}
\newcommand{\QueryDist}[1]{\mathrm{Query}(#1)}
\newcommand{\AllDist}{DistGen_1}
\newcommand{\Diff}{\sets{Diff}}


\newcommand{\dhat}[1]{\wh{\wh{#1}}}


\newcommand{\tmclass}{\fclass}
\newcommand{\Sim}{\mathsf{Sim}}
\newcommand{\ext}{^{\mathsf{ext}}}

\newcommand{\MSK}{\mathsf{MSK}}
\newcommand{\MPK}{\mathsf{MPK}}
\newcommand{\ID}{f}
\newcommand{\nand}{\barwedge}

\newcommand{\fclass}{\cF}
\newcommand{\secp}{\mathrm{\kappa}}
\newcommand{\secpar}{\secp}

%\newcommand{\Samp}{\mathsf{OnSam}}

\newcommand{\Sam}{\mathsf{Sam}}

%\newcommand{\Att}{\textsc{Attack}}
\newcommand{\Hyb}{\textsc{Hybrid}}
\newcommand{\Idl}{\textsc{Ideal}}
\newcommand{\Lzy}{\textsc{Lazy}}

\newcommand{\HIT}{\mathsf{HIT}}
\newcommand{\MAL}{\mathsf{MAL}}
\newcommand{\INT}{\mathsf{INT}}

\newcommand{\sm}{\setminus}
%\newcommand{\att}{_\mathsf{att}}
\newcommand{\hyb}{_\mathsf{hyb}}
\newcommand{\idl}{_\mathsf{idl}}

\newcommand{\oAtt}{\mathbf{Out}\att}
\newcommand{\oHyb}{\mathbf{Out}\hyb}
\newcommand{\oIdl}{\mathbf{Out}\idl}

\newcommand{\bHyb}{B_\mathsf{hyb}}
\newcommand{\bAtt}{B_\mathsf{att}}
\newcommand{\todo}[1]{{\bf \textcolor{red}{#1}}}
\newcommand{\Chal}{\mathsf{Chal}}
\newcommand{\gen}{\mathbf{gen}}

\newcommand{\Clsr}{\CLSR}

\newcommand{\OR}{\mathsf{OR}}
\newcommand{\AND}{\mathsf{AND}}

\newcommand{\BadE}{\mathsf{BE}} % bad event
\newcommand{\model}{h}
\newcommand{\modelD}[1]{\model_{-#1}}
\newcommand{\modelDel}{\model_{\mathsf{del}}}
\newcommand{\del}{\mathsf{del}}
% keys mathsf
\newcommand{\sk}{\mathsf{sk}}
\newcommand{\SK}{\mathsf{SK}}
\newcommand{\pk}{\mathsf{pk}}
\newcommand{\PK}{\mathsf{PK}}
\newcommand{\dk}{\mathsf{dk}}
\newcommand{\DK}{\mathsf{DK}}
\newcommand{\problem}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\Rplus}{\R_+}
\newcommand{\Loss}{\mathsf{Loss}}
\newcommand{\loss}{\ell}
% algorithms mahtbf
\newcommand{\e}{\mathrm{e}}
\newcommand{\E}{\mathrm{E}}
\renewcommand{\d}{\mathbf{d}}
\newcommand{\id}{\mathbf{id}}
\newcommand{\g}{\mathbf{g}}
% \newcommand{\G}{\mathbf{G}}
\renewcommand{\k}{\mathbf{k}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\p}{\mathbf{p}}


\newcommand{\clg}{\ol{\g}}
\newcommand{\clk}{\ol{\k}}
\newcommand{\clid}{\ol{\id}}
\newcommand{\cle}{\ol{\e}}
\newcommand{\cld}{\ol{\d}}



% sets
\newcommand{\atA}{\mathbb{A}}
\newcommand{\atB}{\mathbb{B}}

\newcommand{\prF}{\mathbb{F}}
\newcommand{\prG}{\mathbb{G}}


\newcommand{\PE}{\mathbf{PE}}
\newcommand{\TPE}{\mathbf{TPE}}
\newcommand{\IBE}{\mathbf{IBE}}
\newcommand{\FPE}{\prF\text{-}\PE}
\newcommand{\GPE}{\prG\text{-}\PE}
\newcommand{\tTPE}{\tau\text{-}\TPE}
\newcommand{\ttTPE}{$\tau$-TPE\xspace}

%\newcommand{\att}{\cA}
%\newcommand{\prd}{\cP}
\usepackage{graphicx}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
\newcommand{\remove}[1]{}
\newcommand{\num}[1]{{\bf (#1)}}

\newcommand{\ol}{\overline}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\nin}{\not \in}

\newcommand{\es}{\varnothing} % empty set
\newcommand{\se}{\subseteq}
\newcommand{\nse}{\not \se}
\newcommand{\nf}[2]{\nicefrac{#1}{#2}}
\newcommand{\rv}[1]{\mathbf{#1}} % Random Variable
\newcommand{\rvV}{\rv{V}}




%%%  English %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etal}{et~al.\ }
\newcommand{\aka}{also known as,\ }
\newcommand{\resp}{resp.,\ }
\newcommand{\ie}{i.e.,\ }
\newcommand{\wolog}{w.l.o.g.\ }
\newcommand{\Wolog}{W.l.o.g.\ }
\newcommand{\eg}{e.g.,\ }
\newcommand{\wrt} {with respect to\ }
\newcommand{\cf}{{cf.,\ }}

%%%  math %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\round}[1]{\lfloor #1 \rceil}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\angles}[1]{\langle #1 \rangle}
\newcommand{\parens}[1]{( #1 )}
\newcommand{\bracks}[1]{[ #1 ]}
\newcommand{\bra}[1]{\langle#1\rvert}
\newcommand{\ket}[1]{\lvert#1\rangle}
\newcommand{\set}[1]{\{ #1 \}}
\newcommand{\Set}[1]{\left\{ #1 \right\}}
\newcommand{\adjRound}[1]{\left\lfloor #1 \right\rceil} % Adjusted Round
\newcommand{\adjCeil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\adjFloor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\adjAngles}[1]{\left\langle #1 \right\rangle}
\newcommand{\adjParens}[1]{\left( #1 \right)}
\newcommand{\adjBracks}[1]{\left[ #1 \right]}
\newcommand{\adjBra}[1]{\left\langle#1\right\rvert}
\newcommand{\adjKet}[1]{\left\lvert#1\right\rangle}
\newcommand{\adjSet}[1]{\left\{ #1 \right\}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\third}{\tfrac{1}{3}}
\newcommand{\quarter}{\tfrac{1}{4}}
\newcommand{\eqdef}{:=}
\newcommand{\zo}{\{0,1\}}
\newcommand{\oo}{\{\pm 1\}}
\newcommand{\bits}{\{0,1\}}
\newcommand{\xor}{\oplus}
\newcommand{\tensor}{\otimes}
\newcommand{\getsr}{\mathbin{\stackrel{\mbox{\,\tiny \$}}{\gets}}}
\newcommand{\from}{\gets}
\newcommand{\size}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\size{#1}}
%\newcommand{\norm}[1]{\abf{#1}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\To}{\mapsto}
\newcommand{\mcom}{\, ,}
\newcommand{\mper}{\, .}
\newcommand{\sign}{\ensuremath {\pm 1}}
\newcommand{\nbyn}{\ensuremath {n \times n}}
\renewcommand{\L}{\ensuremath L\:}
\newcommand{\LA}{\ensuremath L_A}

%%%% Font Abbreviations

\newcommand{\R}{{\mathbb R}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\F}{{\mathbb F}}

\newcommand{\trainTam}{\vVec}
\newcommand{\Adv}{\mathsf{Adv}}

\newcommand{\train}{\uVec}
\newcommand{\tamped}[1]{\wh{#1}}

\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}


\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

\usepackage{upgreek}
\usepackage{bm}

% note the short forms: eps and ups
\newcommand{\bfalpha}{{\bm \alpha}}
\newcommand{\bfbeta}{{\bm \beta}}
\newcommand{\bfgamma}{{\bm \gamma}}
\newcommand{\bfdelta}{{\bm \delta}}
\newcommand{\bfeps}{{\bm \epsilon}}
\newcommand{\bfveps}{{\bm \varepsilon}}
\newcommand{\bfzeta}{{\bm \zeta}}
\newcommand{\bftheta}{{\bm \theta}}
\newcommand{\bfvtheta}{{\bm \vartheta}}
\newcommand{\bfiota}{{\bm \iota}}
\newcommand{\bfkappa}{{\bm \kappa}}
\newcommand{\bflambda}{{\bm \lambda}}
\newcommand{\bfmu}{{\bm \mu}}
\newcommand{\bfnu}{{\bm \nu}}
\newcommand{\bfxi}{{\bm \xi}}
\newcommand{\bfoo}{{\bm \o}}% not to confuse with regular o
\newcommand{\bfpi}{{\bm \pi}}
\newcommand{\bfvarpi}{{\bm \varpi}}
\newcommand{\bfrho}{{\bm \rho}}
\newcommand{\bfvrho}{{\bm \varrho}}
\newcommand{\bfsigma}{{\bm \sigma}}
\newcommand{\bfvsigma}{{\bm \varsigma}}
\newcommand{\bftau}{{\bm \tau}}
\newcommand{\bfups}{{\bm \upsilon}}
\newcommand{\bfphi}{{\bm \phi}}
\newcommand{\bfvphi}{{\bm \varphi}}
\newcommand{\bfchi}{{\bm \chi}}
\newcommand{\bfpsi}{{\bm \psi}}
\newcommand{\bfomega}{{\bm \omega}}


\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfU}{\mathsf{U}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}

\newcommand{\sfa}{\mathsf{a}}
\newcommand{\sfb}{\mathsf{b}}
\newcommand{\sfc}{\mathsf{c}}
\newcommand{\sfd}{\mathsf{d}}
\newcommand{\sfe}{\mathsf{e}}
\newcommand{\sff}{\mathsf{f}}
\newcommand{\sfg}{\mathsf{g}}
\newcommand{\sfh}{\mathsf{h}}
\newcommand{\sfi}{\mathsf{i}}
\newcommand{\sfj}{\mathsf{j}}
\newcommand{\sfk}{\mathsf{k}}
\newcommand{\sfl}{\mathsf{l}}
\newcommand{\sfm}{\mathsf{m}}
\newcommand{\sfn}{\mathsf{n}}
\newcommand{\sfo}{\mathsf{o}}
\newcommand{\sfp}{\mathsf{p}}
\newcommand{\sfq}{\mathsf{q}}
\newcommand{\sfr}{\mathsf{r}}
\newcommand{\sfs}{\mathsf{s}}
\newcommand{\sft}{\mathsf{t}}
\newcommand{\sfu}{\mathsf{u}}
\newcommand{\sfv}{\mathsf{v}}
\newcommand{\sfw}{\mathsf{w}}
\newcommand{\sfx}{\mathsf{x}}
\newcommand{\sfy}{\mathsf{y}}
\newcommand{\sfz}{\mathsf{z}}
\newcommand{\eps}{\varepsilon}
%\newcommand{\e}{\epsilon}
\newcommand{\veps}{\varepsilon}
%\newcommand{\vare}{\varepsilon}
\newcommand{\vphi}{\varphi}
\newcommand{\vsigma}{\varsigma}
\newcommand{\vrho}{\varrho}
\newcommand{\vpi}{\varpi}
\newcommand{\tO}{\widetilde{O}}
\newcommand{\tOmega}{\widetilde{\Omega}}
\newcommand{\tTheta}{\widetilde{\Theta}}
\newcommand{\field}{\ensuremath \Bbbk}
\newcommand{\reals}{\ensuremath \mathbb{R}}
\DeclareMathOperator{\Rig}{Rig}
\DeclareMathOperator{\rk}{rank}

\DeclareMathOperator{\rank}{rank}

%%%%%%%%%%%%%%%% Operators %%%%%%

\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\loglog}{\operatorname{loglog}}
\newcommand{\GF}{\operatorname{GF}}
\newcommand{\Exp}{\operatorname*{\mathbb{E}}}
\newcommand{\Ex}{\Exp}
\newcommand{\View}{\operatorname{View}}
%\newcommand{\View}[1]{\mathsf{View}\angles{#1}}
\newcommand{\Var}{\operatorname*{\mathbb{V}}}
\newcommand{\ShH}{\operatorname{H}}
\newcommand{\maxH}{\operatorname{H_0}}
\newcommand{\minH}{\operatorname{H_{\infty}}}
\newcommand{\Enc}{\operatorname{Enc}}
\newcommand{\Setup}{\operatorname{Setup}}
\newcommand{\KGen}{\operatorname{KGen}}
\newcommand{\Dec}{\operatorname{Dec}}
\newcommand{\Sign}{\operatorname{Sign}}
\newcommand{\Ver}{\operatorname{Ver}}
\newcommand{\Gen}{\operatorname{Gen}}
\newcommand{\negl}{\operatorname{negl}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\maj}{\operatorname*{maj}}
\newcommand{\argmax}{\operatorname*{argmax}}
\newcommand{\argmin}{\operatorname*{argmin}}
\newcommand{\Image}{\operatorname{Im}}


%%% Computational Problems %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\SAT}{\mathrm{SAT}}
\newcommand{\UNSAT}{\mathrm{UNSAT}}
%\newcommand{\ED}{\mathrm{ED}} % Entropy Difference
%\newcommand{\GapSVP}{\mathrm{GapSVP}}
%\newcommand{\GapSIVP}{\mathrm{GapSIVP}}
%\newcommand{\GapCVP}{\mathrm{GapCVP}}
%\newcommand{\COLOR}{\mathrm{3COL}}

%%% Complexity Classes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\class}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\coclass}[1]{\class{co\mbox{-}#1}} %  their complements
\newcommand{\prclass}[1]{\class{Pr#1}}
\newcommand{\PPT}{\class{PPT}}
\newcommand{\BPP}{\class{BPP}}
\newcommand{\NC}{\class{NC}}
\newcommand{\AC}{\class{AC}}
\newcommand{\NP}{\ensuremath{\class{NP}}}
\newcommand{\coNP}{\ensuremath{\coclass{NP}}}
\newcommand{\RP}{\class{RP}}
\newcommand{\coRP}{\coclass{RP}}
\newcommand{\ZPP}{\class{ZPP}}
\newcommand{\IP}{\class{IP}}
\newcommand{\coIP}{\coclass{IP}}
\newcommand{\AM}{\class{AM}}
\newcommand{\coAM}{\class{coAM}}
\newcommand{\MA}{\class{MA}}
\renewcommand{\P}{\class{P}}
\newcommand\prBPP{\prclass{BPP}}
\newcommand\prRP{\prclass{RP}}
%\newcommand\prP{\prclass{P}}
\newcommand{\Ppoly}{\class{P/poly}}
\newcommand{\DTIME}{\class{DTIME}}
\newcommand{\ETIME}{\class{E}}
\newcommand{\BPTIME}{\class{BPTIME}}
\newcommand{\AMTIME}{\class{AMTIME}}
\newcommand{\coAMTIME}{\class{coAMTIME}}
\newcommand{\NTIME}{\class{NTIME}}
\newcommand{\coNTIME}{\class{coNTIME}}
\newcommand{\AMcoAM}{\class{AM} \cap \class{coAM}}
\newcommand{\NPcoNP}{\class{N} \cap \class{coN}}
\newcommand{\EXP}{\class{EXP}}
\newcommand{\SUBEXP}{\class{SUBEXP}}
\newcommand{\qP}{\class{\wt{P}}}
\newcommand{\PH}{\class{PH}}
\newcommand{\NEXP}{\class{NEXP}}
\newcommand{\PSPACE}{\class{PSPACE}}
%\newcommand{\E}{\class{E}}
\newcommand{\one}{\vmathbb{1}}
\newcommand{\NE}{\class{NE}}
\newcommand{\coNE}{\class{coNE}}
\newcommand{\SharpP}{\class{\#P}}
\newcommand{\prSZK}{\prclass{SZK}}
\newcommand{\BPPSZK}{\BPP^{\SZK}}
\newcommand{\TFAM}{\class{TFAM}}
\newcommand{\RTFAM}{{\R\text{-}\class{TUAM}}}
% relations decidable by a randomized algorithm
\newcommand{\FBPP}{\class{BPP}}
% relations decidable by a RTFAM oracle
\newcommand{\BPPR}{\FBPP^{\RTFAM}}
\newcommand{\TFNP}{\mathbf{TFNP}}
\newcommand{\MIP}{\mathbf{MIP}}
% zero-knowledge complexity classes
\newcommand{\ZK}{\class{ZK}}
\newcommand{\SZK}{\class{SZK}}
\newcommand{\SZKP}{\class{SZKP}}
\newcommand{\SZKA}{\class{SZKA}}
\newcommand{\CZKP}{\class{CZKP}}
\newcommand{\CZKA}{\class{CZKA}}
\newcommand{\coSZKP}{\coclass{SZKP}}
\newcommand{\coSZKA}{\coclass{SZKA}}
\newcommand{\coCZKP}{\coclass{CZKP}}
\newcommand{\coCZKA}{\coclass{CZKA}}
\newcommand{\NISZKP}{\class{NI\mbox{-}SZKP}}
\newcommand{\phcc}{\ensuremath \PH^{\mathrm{cc}}}
\newcommand{\pspacecc}{\ensuremath \PSPACE^{\mathrm{cc}}}
\newcommand{\sigcc}[1]{\ensuremath \class{\Sigma}^{\mathrm{cc}}_{#1}}
\newcommand{\aco}{\ensuremath \AC^0}
\newcommand{\ncone}{\ensuremath \NC^1}

%%%%% Theorem environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\ifllncs
\newtheorem{aclaim}{Claim}
%\fi



\newtheorem{theorem}{Theorem}[section]
\newtheorem{inftheorem}{Informal Theorem}[section]
\theoremstyle{plain}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
\theoremstyle{definition}

\newtheorem{definition/}[theorem]{Definition}
\newenvironment{definition}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{definition/}}
  {\popQED\end{definition/}}
\newtheorem{infdefinition}[theorem]{Informal Definition}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{alg/}[theorem]{Algorithm}

\newenvironment{alg}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{alg/}}
  {\popQED\end{alg/}}
  
\newtheorem{example}[theorem]{Example}
\newtheorem{algorithm1}[theorem]{Algorithm}
%\newtheorem{protocol}[theorem]{Protocol} defined below
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
% \newtheorem{note}[theorem]{Note}

\newenvironment{proofof}[1]{\begin{proof}[\textit{Proof of #1}]}{\end{proof}}
\newenvironment{proofsketch}{\begin{proof}[\textit{Proof Sketch}]}{\end{proof}}
\newenvironment{proofsketchof}[1]{\begin{proof}[\textit{Proof Sketch of #1}]}{\end{proof}}

% Protocol env
\newcommand{\sdotfill}{\textcolor[rgb]{0.8,0.8,0.8}{\dotfill}} %change to \cdotfill later
\newenvironment{protocol}{\begin{proto}}{\vspace{-\topsep}\sdotfill\end{proto}}

\makeatletter
\def\th@protocol{%
    \normalfont % body font
    \setbeamercolor{block title example}{bg=orange,fg=white}
    \setbeamercolor{block body example}{bg=orange!20,fg=black}
    \def\inserttheoremblockenv{exampleblock}
  }
\makeatother
\theoremstyle{protocol}

\newtheorem{proto}[theorem]{Protocol}
\newtheorem{protoc}[theorem]{Protocol}
\newenvironment{protocolS}{\begin{protoc}}{\vspace{-\topsep}\sdotfill\end{protoc}}

% state/restate
\newcommand{\namedref}[2]{#1~\ref{#2}}

\newcommand{\torestate}[3]{%
\expandafter \def \csname BBRESTATE #2 \endcsname{#3}
\theoremstyle{plain}
\newtheorem{BBRESTATETHMNUM#2}[theorem]{#1}
\begin{BBRESTATETHMNUM#2}\label{#2}\csname BBRESTATE #2 \endcsname   \end{BBRESTATETHMNUM#2}
\newtheorem*{BBRESTATETHMNONNUM#2}{\namedref{#1}{#2}}
}

\newcommand{\restate}[1]{\begin{BBRESTATETHMNONNUM#1}[Restated] \csname BBRESTATE #1 \endcsname
\end{BBRESTATETHMNONNUM#1}}

%%% refs macros (hopefully will help in transforming to pdf) %%%%%%


\newcommand{\theoremref}[1]{Theorem~\ref{#1}}
\newcommand{\sectionref}[1]{Sect.~\ref{#1}}
\newcommand{\definitionref}[1]{Definition~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\stepref}[1]{Step~\ref{#1}}
\newcommand{\figureref}[1]{Fig.~\ref{#1}}
\newcommand{\lemmaref}[1]{Lemma~\ref{#1}}
\newcommand{\claimref}[1]{Claim~\ref{#1}}
\newcommand{\remarkref}[1]{Remark~\ref{#1}}
\newcommand{\corollaryref}[1]{Corollary~\ref{#1}}
\newcommand{\inequalityref}[1]{Inequality~\ref{#1}}
\newcommand{\constructionref}[1]{Construction~\ref{#1}}
\newcommand{\itemref}[1]{Item~\ref{#1}}
\newcommand{\propertyref}[1]{Property~\ref{#1}}
\newcommand{\protocolref}[1]{Protocol~\ref{#1}}
\newcommand{\algorithmref}[1]{Algorithm~\ref{#1}}
\newcommand{\appendixref}[1]{Appendix~\ref{#1}}


% More shorthand

\newcommand{\ra}{\rightarrow}
\newcommand{\approxmd}{\approx^{\infty}}
\newcommand{\simgame}{\mathsf{SimGame}}
\newcommand{\avgsimgame}{\mathsf{AvgSimGame}}

% From GGV
\newcommand{\state}         {\mathnormal{state}} 
\newcommand{\view}          {\mathnormal{view}}


\newcommand{\wght}{\mathsf{wt}}
\newcommand{\comp}{\mathsf{comp}}
